Sampling of Signals on Multigraphs: From Removable and Uniqueness sets to Spectral Proxies

In this paper, we study the sampling of bandlimited signals on multigraphs, where several graphs with different shift operators are defined on the same set of nodes. Since the shift operators do not commute in general, they admit only a joint block diagonalization, and the frequencies of the multigraph signal model are matrices rather than scalars. Relying on a formal algebraic convolutional signal model, we introduce a notion of frequency and bandwidth for multigraph signals that does not depend on any individual layer, and we extend the notions of removable and uniqueness sets to multigraphs. We prove that the optimality of a sampling set is determined exclusively by the common Fourier basis and its invariant subspaces, and not by any individual layer, although the individual layers provide computable sufficient conditions that certify a sampling set as a uniqueness set. Since identifying which layers provide reliable certificates requires spectral information, we propose an aggregate operator that pools the information of all the layers, is computable directly from the shift operators, and certifies uniqueness without any assumption on the individual layers. This operator leads to a greedy sampling algorithm that does not require computing the joint block diagonalization. Numerical experiments on multigraphs whose layers order the frequencies inconsistently show that the proposed algorithm selects better-conditioned sampling sets and attains lower reconstruction errors than single-layer methods.

==> figures/experiments/asp_pgfplots_style.tex <==
% ASP Lab pgfplots style for the multigraph sampling figures (generated by make_paper_tikz.py).
% Preamble requirements:
%   \usepackage{pgfplots} \usepgfplotslibrary{groupplots,fillbetween}
%   \usetikzlibrary{calc} \pgfplotsset{compat=1.18}
\def\aspstyleloaded{}
\definecolor{aspnavy}{HTML}{0A1628}
\definecolor{aspgold}{HTML}{A8862B}
\definecolor{asplayer}{HTML}{3D5A8A}
\definecolor{asprandom}{HTML}{BDBDBD}
\definecolor{aspmuted}{HTML}{4A4A4A}
\definecolor{aspgrid}{HTML}{E4E4E4}
\pgfplotsset{
  asp axis/.style={
    scale only axis,
    axis lines*=left,
    axis line style={aspmuted, line width=0.6pt},
    every tick/.style={aspmuted, line width=0.5pt},
    xmajorgrids, ymajorgrids,
    major grid style={aspgrid, line width=0.5pt},
    font=\footnotesize,
    tick label style={font=\scriptsize, text=aspmuted},
    label style={font=\footnotesize},
    title style={font=\footnotesize, yshift=-3pt},
    clip mode=individual,
  },
  asp log/.style={ymode=log, log basis y=10},
  asp legend/.style={
    legend columns=-1,
    legend cell align=left,
    legend style={draw=none, fill=none, font=\scriptsize,
                  /tikz/every even column/.append style={column sep=10pt}},
  },
  sm1/.style={aspnavy, line width=1.8pt, mark=*, mark size=2pt,
              mark options={solid, fill=aspnavy, line width=0.8pt}},
  sm2best/.style={asplayer, line width=1.4pt, dash pattern=on 6pt off 2pt on 1.5pt off 2pt,
                  mark=triangle*, mark size=2.4pt, mark options={solid, fill=asplayer, line width=0.8pt}},
  sm2band/.style={draw=none, fill=asplayer, fill opacity=0.18},
  sm3/.style={aspgold, line width=1.6pt, dash pattern=on 8pt off 3.2pt,
              mark=square*, mark size=1.9pt, mark options={solid, fill=aspgold, line width=0.8pt}},
  sm4/.style={asprandom, line width=1.8pt, dash pattern=on 1.8pt off 2.7pt,
              mark=x, mark size=2.4pt, mark options={solid, line width=0.8pt}},
}
\tikzset{refline/.style={aspmuted, line width=0.6pt, dash pattern=on 0.6pt off 1.6pt}}


==> figures/fig13_tikz_source.tex <==
%!TEX root = fig13_standalone.tex








%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Primary Colors of the Palette
\definecolor{my_alejocol5}{RGB}{1,31,75}
\definecolor{my_alejocol4}{RGB}{3,57,108}
\definecolor{my_alejocol3}{RGB}{0,91,150}
\definecolor{my_alejocol2}{RGB}{100,151,177}
\definecolor{my_alejocol1}{RGB}{179,205,224}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}

%--------Secondary Colors of the Palette
\definecolor{my_alejocol4s}{RGB}{212, 220, 220}
\definecolor{my_alejocol3s}{RGB}{113, 18, 55}
\definecolor{my_alejocol2s}{RGB}{236, 85, 141}
\definecolor{my_alejocol1s}{RGB}{225, 73, 132}


%-- Four colors Color Palette
\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
\definecolor{my_cp4_col4}{RGB}{99, 143, 169}



% Syntax:
% \DoublLine[half of the double line distance]{first node}{second node}{options line 1}{label line 1}{options line 2}{label line 2}
\newcommand\DoubleLine[7][4pt]{%
    \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
    \draw[#4]($(h1)!#1!90:(h2)$)-- node [auto=left] {#5} ($(h2)!#1!-90:(h1)$); 
    \draw[#6]($(h1)!#1!-90:(h2)$)-- node [auto=right] {#7} ($(h2)!#1!90:(h1)$);
    }
    


    \begin{tikzpicture}[myn/.style={circle,  thin, draw, inner sep=0.15cm, outer sep=2pt, ball color=my_cp4_col3}]




%%-----------------------------------------
%%---------------- NODES ------------------
%%-----------------------------------------

    % Node
    \node[myn] (s) at (0,2) {$1$};
    % Signal component
    \path (s) + (0,0.8) coordinate (c);
    \node (x1) at (c)  {$\mathbf{x}(1)$};
    
    
    % Node
    \node[myn] (a) at (2,4) {$2$};
    % Signal component
    \path (a) + (0,0.8) coordinate (c);
    \node (x2) at (c)  {$\mathbf{x}(2)$};
    
    
    % Node  
    \node[myn] (b) at (2,0) {$3$};
    % Signal component
    \path (b) + (0,-0.8) coordinate (cx);
    \node (x3) at (cx)  {$\mathbf{x}(3)$};
    
    
    % Node  
    \node[myn] (c) at (5,4) {$4$};
    % Signal component
     \path (c) + (0,0.8) coordinate (cx);
     \node (x4) at (cx)  {$\mathbf{x}(4)$};
    
    
    % Node
    \node[myn] (d) at (5,0) {$5$};
    % Signal component
     \path (d) + (0,-0.8) coordinate (cx);
     \node (x5) at (cx)  {$\mathbf{x}(5)$};
    
    
    % Node
    \node[myn] (t) at (7,2) {$6$};
    % Signal component
    \path (t) + (0,0.8) coordinate (cx);
    \node (x6) at (cx)  {$\mathbf{x}(6)$};
    


%%-----------------------------------------------------
%%---------------- Shiftrs Operators ------------------
%%-----------------------------------------------------


%\node[myn] (a) at (2,4) {$2$};
% Signal component
\path (a) + (-1.5,0.8) coordinate (caux);
\node[color=my_cp4_col2] at (caux)  { $\mathbf{S}_{1}\rightarrow \mathcal{E}_1$ };

\path (d) + (1.5,-0.8) coordinate (caux);
\node[color=my_cp4_col1] at (caux)  { $\mathbf{S}_{2}\rightarrow \mathcal{E}_2$ };


%%-----------------------------------------
%%-------------- EDGES ------------------
%%-----------------------------------------

    \DoubleLine{s}{a}{-,very thick, my_cp4_col2}{1}{-,very thick, my_cp4_col1}{7}
    \DoubleLine{s}{b}{-,very thick, my_cp4_col2}{2}{-,very thick, my_cp4_col1}{6}
    \DoubleLine{a}{b}{-,very thick, my_cp4_col2}{3}{-,very thick, my_cp4_col1}{5}
    \DoubleLine{a}{c}{-,very thick, my_cp4_col2}{4}{-,very thick, my_cp4_col1}{4}
    \DoubleLine{b}{d}{-,very thick, my_cp4_col2}{5}{-,very thick, my_cp4_col1}{3}
    \DoubleLine{c}{t}{-,very thick, my_cp4_col2}{6}{-,very thick, my_cp4_col1}{2}
    \DoubleLine{d}{t}{-,very thick, my_cp4_col2}{7}{-,very thick, my_cp4_col1}{1}
    \DoubleLine{c}{d}{-,very thick, my_cp4_col2}{7}{-,very thick, my_cp4_col1}{1}
    
   % \draw[color=red] (a) -- (dd) 


    \end{tikzpicture}





==> figures/fig_14_tikz_source.tex <==
%!TEX root = fig_14_standalone.tex








%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Primary Colors of the Palette
\definecolor{my_alejocol5}{RGB}{1,31,75}
\definecolor{my_alejocol4}{RGB}{3,57,108}
\definecolor{my_alejocol3}{RGB}{0,91,150}
\definecolor{my_alejocol2}{RGB}{100,151,177}
\definecolor{my_alejocol1}{RGB}{179,205,224}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}

%--------Secondary Colors of the Palette
\definecolor{my_alejocol4s}{RGB}{212, 220, 220}
\definecolor{my_alejocol3s}{RGB}{113, 18, 55}
\definecolor{my_alejocol2s}{RGB}{236, 85, 141}
\definecolor{my_alejocol1s}{RGB}{225, 73, 132}






%%-- Four colors Color Palette
%\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
%\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
%\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
%\definecolor{my_cp4_col4}{RGB}{99, 143, 169}

\definecolor{my_cp4_col1}{RGB}{110,142,187}
\definecolor{my_cp4_col2}{RGB}{182,103,105}
\definecolor{my_cp4_col3}{RGB}{135,169,107}
\definecolor{my_cp4_col4}{RGB}{219,167,108}


%Dark Blue: #6e8ebb, rgba(110,142,187,255)
%Dark Red: #b66769, rgba(182,103,105,255)
%Dark Green: #87a96b, rgba(135,169,107,255)
%Dark Yellow:  #dba76c, rgba(219,167,108,255)


%-----------------------
%------ Scale ----------
%-----------------------

\def \scale {2}
\def \unit  { \scale cm}

% Scale for the images
\def \moviescale{0.05}









% Syntax:
% \DoublLine[half of the double line distance]{first node}{second node}{options line 1}{label line 1}{options line 2}{label line 2}
\newcommand\DoubleLine[7][4pt]{%
    \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
    \draw[#4]($(h1)!#1!90:(h2)$)-- node [auto=left] {#5} ($(h2)!#1!-90:(h1)$); 
    \draw[#6]($(h1)!#1!-90:(h2)$)-- node [auto=right] {#7} ($(h2)!#1!90:(h1)$);
    }
    


    \begin{tikzpicture}[myn/.style={circle,  thin, draw, inner sep=0.15cm, outer sep=2pt, ball color=my_cp4_col3}]




%%------- XY Coordinates to Locate Movies -------

%    1.0000         0
%    0.7071    0.7071
%    0.0000    1.0000
%    -0.7071    0.7071
%    -1.0000    0.0000
%    -0.7071   -0.7071
%    -0.0000   -1.0000
%    0.7071   -0.7071




%%--------------------------------------------------
%%------------ ADDING THE MOVIES --------------
%%--------------------------------------------------

% Movie
\node[inner sep=0pt] (movie1) at (1*\unit,0*\unit) 
{\includegraphics[width=\moviescale\textwidth]{./external_images/movie_1}};
% Signal
\path (1.5*\unit,0*\unit) coordinate (c);
\node (x1) at (c)  {$\mathbf{x}(1)$};


% Movie
\node[inner sep=0pt] (movie2) at (0.7071*\unit,0.7071*\unit)
{\includegraphics[width=\moviescale\textwidth]{./external_images/movie_2}};
% Signal 
\path (1.5*0.7071*\unit,1.5*0.7071*\unit) coordinate (c);
\node (x2) at (c)  {$\mathbf{x}(2)$};


% Movie
\node[inner sep=0pt] (movie3) at (0*\unit,1*\unit)
{\includegraphics[width=\moviescale\textwidth]{./external_images/movie_3}};
% Signal
\path (0*\unit,1.5*\unit) coordinate (c);
\node (x3) at (c)  {$\mathbf{x}(3)$};


% Movie
\node[inner sep=0pt] (movie4) at (-0.7071*\unit,0.7071*\unit)
{\includegraphics[width=\moviescale\textwidth]{./external_images/movie_4}};
% Signal
\path (-1.5*0.7071*\unit,1.5*0.7071*\unit) coordinate (c);
\node (x4) at (c)  {$\mathbf{x}(4)$};


% Movie
\node[inner sep=0pt] (movie5) at (-1*\unit,0*\unit)
{\includegraphics[width=\moviescale\textwidth]{./external_images/movie_5}};
% Signal
\path (-1.5*\unit,0*\unit) coordinate (c);
\node (x5) at (c)  {$\mathbf{x}(5)$};


% Movie
\node[inner sep=0pt] (movie6) at (-0.7071*\unit,-0.7071*\unit)
{\includegraphics[width=\moviescale\textwidth]{./external_images/movie_6}};
% Signal 
\path (-1.5*0.7071*\unit,-1.5*0.7071*\unit) coordinate (c);
\node (x6) at (c)  {$\mathbf{x}(6)$};


% Movie
\node[inner sep=0pt] (movie7) at (0*\unit,-1*\unit)
{\includegraphics[width=\moviescale\textwidth]{./external_images/movie_7}};
% Signal
\path (0*\unit,-1.5*\unit) coordinate (c);
\node (x7) at (c)  {$\mathbf{x}(7)$};


% Movie
\node[inner sep=0pt] (movie8) at (0.7071*\unit,-0.7071*\unit)
{\includegraphics[width=\moviescale\textwidth]{./external_images/movie_8}};
% Signal
\path (1.5*0.7071*\unit,-1.5*0.7071*\unit) coordinate (c);
\node (x8) at (c)  {$\mathbf{x}(8)$};






%%-----------------------------------------------------------
%%--------- DRAWING THE MULTIGRAPH EDGES  ----------
%%-----------------------------------------------------------


%%----- From Node 1 to ------

\path (movie1) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (movie2);
%\path (movie1) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie3);
%\path (movie1) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie4);
\path (movie1) edge  [bend right, line width=1, color=my_cp4_col2, opacity=0.6] node {} (movie5);
\path (movie1) edge  [bend right, line width=1, color=my_cp4_col3, opacity=0.6] node {} (movie6);
\path (movie1) edge  [bend right, line width=1, color=my_cp4_col4, opacity=0.6] node {} (movie7);
\path (movie1) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (movie8);


%%----- From Node 2 to ------

\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2, opacity=0.6] node {} (movie3);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie4);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie5);
\path (movie2) edge  [bend right, line width=1, color=my_cp4_col3, opacity=0.6] node {} (movie6);
\path (movie2) edge  [bend right, line width=1, color=my_cp4_col4, opacity=0.6] node {} (movie7);
\path (movie2) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (movie8);
\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2, opacity=0.6] node {} (movie1);



%%----- From Node 3 to ------

\path (movie3) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (movie4);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie4);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie5);
\path (movie3) edge  [bend right, line width=1, color=my_cp4_col2, opacity=0.6] node {} (movie7);
\path (movie3) edge  [bend right, line width=1, color=my_cp4_col3, opacity=0.6] node {} (movie8);
\path (movie3) edge  [bend right, line width=1, color=my_cp4_col4, opacity=0.6] node {} (movie1);
\path (movie3) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (movie2);



%%----- From Node 4 to ------

\path (movie4) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (movie5);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie4);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie5);
\path (movie4) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (movie8);
\path (movie4) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (movie1);
\path (movie4) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (movie2);
\path (movie4) edge  [bend right, line width=1, color=my_cp4_col2,,opacity=0.6] node {} (movie3);




%%----- From Node 5 to ------

\path (movie5) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (movie6);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie4);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie5);
\path (movie5) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (movie1);
\path (movie5) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (movie2);
\path (movie5) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (movie3);
\path (movie5) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (movie4);



%%----- From Node 6 to ------

\path (movie6) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (movie7);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie4);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie5);
\path (movie6) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (movie2);
\path (movie6) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (movie3);
\path (movie6) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (movie4);
\path (movie6) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (movie5);



%%----- From Node 7 to ------

\path (movie7) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (movie8);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie4);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie5);
\path (movie7) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (movie3);
\path (movie7) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (movie4);
\path (movie7) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (movie5);
\path (movie7) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (movie6);



%%----- From Node 8 to ------

\path (movie8) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (movie1);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie4);
%\path (movie2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (movie5);
\path (movie8) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (movie4);
\path (movie8) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (movie5);
\path (movie8) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (movie6);
\path (movie8) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (movie7);





    \end{tikzpicture}





==> figures/fig_19_tikz_source.tex <==
%!TEX root = fig_14_standalone.tex








%%%%%%%%%%%%%%%%%%%%%%% Colors %%%%%%%%%%%%%%%%%%%%

%%-------Primary Colors of the Palette
\definecolor{my_alejocol5}{RGB}{1,31,75}
\definecolor{my_alejocol4}{RGB}{3,57,108}
\definecolor{my_alejocol3}{RGB}{0,91,150}
\definecolor{my_alejocol2}{RGB}{100,151,177}
\definecolor{my_alejocol1}{RGB}{179,205,224}

%--Gray colors added to the pallette
\colorlet{my_alejocolg1}{black!30}
\colorlet{my_alejocolg2}{black!35}
\colorlet{my_alejocolg3}{black!40}
\colorlet{my_alejocolg4}{black!45}
\colorlet{my_alejocolg5}{black!50}
\colorlet{my_alejocolg6}{black!55}
\colorlet{my_alejocolg7}{black!60}

%--------Secondary Colors of the Palette
\definecolor{my_alejocol4s}{RGB}{212, 220, 220}
\definecolor{my_alejocol3s}{RGB}{113, 18, 55}
\definecolor{my_alejocol2s}{RGB}{236, 85, 141}
\definecolor{my_alejocol1s}{RGB}{225, 73, 132}






%%-- Four colors Color Palette
%\definecolor{my_cp4_col1}{RGB}{255, 86, 87}
%\definecolor{my_cp4_col2}{RGB}{55, 108, 138}
%\definecolor{my_cp4_col3}{RGB}{242, 217, 187}
%\definecolor{my_cp4_col4}{RGB}{99, 143, 169}

\definecolor{my_cp4_col1}{RGB}{110,142,187}
\definecolor{my_cp4_col2}{RGB}{182,103,105}
\definecolor{my_cp4_col3}{RGB}{135,169,107}
\definecolor{my_cp4_col4}{RGB}{219,167,108}


%Dark Blue: #6e8ebb, rgba(110,142,187,255)
%Dark Red: #b66769, rgba(182,103,105,255)
%Dark Green: #87a96b, rgba(135,169,107,255)
%Dark Yellow:  #dba76c, rgba(219,167,108,255)


%-----------------------
%------ Scale ----------
%-----------------------

\def \scale {2}
\def \unit  { \scale cm}

% Scale for the images
\def \imgscale{0.05}









% Syntax:
% \DoublLine[half of the double line distance]{first node}{second node}{options line 1}{label line 1}{options line 2}{label line 2}
\newcommand\DoubleLine[7][4pt]{%
    \path(#2)--(#3)coordinate[at start](h1)coordinate[at end](h2);
    \draw[#4]($(h1)!#1!90:(h2)$)-- node [auto=left] {#5} ($(h2)!#1!-90:(h1)$); 
    \draw[#6]($(h1)!#1!-90:(h2)$)-- node [auto=right] {#7} ($(h2)!#1!90:(h1)$);
    }
    


    \begin{tikzpicture}[myn/.style={circle,  thin, draw, inner sep=0.15cm, outer sep=2pt, ball color=my_cp4_col3}]




%%------- XY Coordinates to Locate Movies -------

%    1.0000         0
%    0.7071    0.7071
%    0.0000    1.0000
%    -0.7071    0.7071
%    -1.0000    0.0000
%    -0.7071   -0.7071
%    -0.0000   -1.0000
%    0.7071   -0.7071




%%--------------------------------------------------
%%------------ ADDING THE MOVIES --------------
%%--------------------------------------------------

% Movie
\node[inner sep=0pt] (img1) at (1*\unit,0*\unit) 
{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_0}};
% Signal
\path (1.5*\unit,0*\unit) coordinate (c);
\node (x1) at (c)  {$\mathbf{x}(1)$};


% Movie
\node[inner sep=0pt] (img2) at (0.7071*\unit,0.7071*\unit)
{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_0}};
% Signal 
\path (1.5*0.7071*\unit,1.5*0.7071*\unit) coordinate (c);
\node (x2) at (c)  {$\mathbf{x}(2)$};


% Movie
\node[inner sep=0pt] (img3) at (0*\unit,1*\unit)
{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_0}};
% Signal
\path (0*\unit,1.5*\unit) coordinate (c);
\node (x3) at (c)  {$\mathbf{x}(3)$};


% Movie
\node[inner sep=0pt] (img4) at (-0.7071*\unit,0.7071*\unit)
{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_0}};
% Signal
\path (-1.5*0.7071*\unit,1.5*0.7071*\unit) coordinate (c);
\node (x4) at (c)  {$\mathbf{x}(4)$};


% Movie
\node[inner sep=0pt] (img5) at (-1*\unit,0*\unit)
{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_0}};
% Signal
\path (-1.5*\unit,0*\unit) coordinate (c);
\node (x5) at (c)  {$\mathbf{x}(5)$};


% Movie
\node[inner sep=0pt] (img6) at (-0.7071*\unit,-0.7071*\unit)
{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_0}};
% Signal 
\path (-1.5*0.7071*\unit,-1.5*0.7071*\unit) coordinate (c);
\node (x6) at (c)  {$\mathbf{x}(6)$};


% Movie
\node[inner sep=0pt] (img7) at (0*\unit,-1*\unit)
{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_0}};
% Signal
\path (0*\unit,-1.5*\unit) coordinate (c);
\node (x7) at (c)  {$\mathbf{x}(7)$};


% Movie
\node[inner sep=0pt] (img8) at (0.7071*\unit,-0.7071*\unit)
{\includegraphics[width=\imgscale\textwidth]{./external_images/Img_0}};
% Signal
\path (1.5*0.7071*\unit,-1.5*0.7071*\unit) coordinate (c);
\node (x8) at (c)  {$\mathbf{x}(8)$};






%%-----------------------------------------------------------
%%--------- DRAWING THE MULTIGRAPH EDGES  ----------
%%-----------------------------------------------------------


%%----- From Node 1 to ------

\path (img1) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (img2);
%\path (img1) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img3);
%\path (img1) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img4);
\path (img1) edge  [bend right, line width=1, color=my_cp4_col2, opacity=0.6] node {} (img5);
\path (img1) edge  [bend right, line width=1, color=my_cp4_col3, opacity=0.6] node {} (img6);
\path (img1) edge  [bend right, line width=1, color=my_cp4_col4, opacity=0.6] node {} (img7);
\path (img1) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (img8);


%%----- From Node 2 to ------

\path (img2) edge  [bend right, line width=1, color=my_cp4_col2, opacity=0.6] node {} (img3);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img4);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img5);
\path (img2) edge  [bend right, line width=1, color=my_cp4_col3, opacity=0.6] node {} (img6);
\path (img2) edge  [bend right, line width=1, color=my_cp4_col4, opacity=0.6] node {} (img7);
\path (img2) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (img8);
\path (img2) edge  [bend right, line width=1, color=my_cp4_col2, opacity=0.6] node {} (img1);



%%----- From Node 3 to ------

\path (img3) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (img4);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img4);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img5);
\path (img3) edge  [bend right, line width=1, color=my_cp4_col2, opacity=0.6] node {} (img7);
\path (img3) edge  [bend right, line width=1, color=my_cp4_col3, opacity=0.6] node {} (img8);
\path (img3) edge  [bend right, line width=1, color=my_cp4_col4, opacity=0.6] node {} (img1);
\path (img3) edge  [bend right, line width=1, color=my_cp4_col1, opacity=0.6] node {} (img2);



%%----- From Node 4 to ------

\path (img4) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (img5);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img4);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img5);
\path (img4) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (img8);
\path (img4) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (img1);
\path (img4) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (img2);
\path (img4) edge  [bend right, line width=1, color=my_cp4_col2,,opacity=0.6] node {} (img3);




%%----- From Node 5 to ------

\path (img5) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (img6);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img4);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img5);
\path (img5) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (img1);
\path (img5) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (img2);
\path (img5) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (img3);
\path (img5) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (img4);



%%----- From Node 6 to ------

\path (img6) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (img7);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img4);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img5);
\path (img6) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (img2);
\path (img6) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (img3);
\path (img6) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (img4);
\path (img6) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (img5);



%%----- From Node 7 to ------

\path (img7) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (img8);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img4);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img5);
\path (img7) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (img3);
\path (img7) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (img4);
\path (img7) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (img5);
\path (img7) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (img6);



%%----- From Node 8 to ------

\path (img8) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (img1);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img4);
%\path (img2) edge  [bend right, line width=1, color=my_cp4_col2] node {} (img5);
\path (img8) edge  [bend right, line width=1, color=my_cp4_col3,opacity=0.6] node {} (img4);
\path (img8) edge  [bend right, line width=1, color=my_cp4_col4,opacity=0.6] node {} (img5);
\path (img8) edge  [bend right, line width=1, color=my_cp4_col1,opacity=0.6] node {} (img6);
\path (img8) edge  [bend right, line width=1, color=my_cp4_col2,opacity=0.6] node {} (img7);





    \end{tikzpicture}





==> figures/tikz_diagrams/fig_5_tikz_source.tex <==



%!TEX root = ../compiler_paper.tex

% ============================================================
% Multigraph figure (3 panels), reusing the K8 layout from the
% original three-graph figure.
%
%   Left panel   : G  = G^(1) \cup G^(2)   (both edge types overlaid)
%   Center panel : G^(1) only  -- 21 edges, "type 1"
%   Right panel  : G^(2) only  --  7 edges, "type 2"
%
% The edge split reuses the exact partition already present in the
% original file's Graph 3 (its 7 commented-out edges = Type 2; the
% remaining 21 active edges = Type 1). Together they form the full
% K8 edge set of Graphs 1/2.
%
% Requires: tikz-network package, and the ASP Lab / Cividis color
% definitions \input{}'d before this file (asp_colors.tex).
% ============================================================

\makeatletter
\newcommand{\gettikzx}[2]{%
	\tikz@scan@one@point\pgfutil@firstofone#1\relax
	\edef#2{\the\pgf@x}%
}
\makeatother

\makeatletter
\newcommand{\gettikzy}[2]{%
	\tikz@scan@one@point\pgfutil@firstofone#1\relax
	\edef#2{\the\pgf@y}%
}
\makeatother

\def\scale{1}
\def\unit{ \scale cm}

% ---------------- Palette assignment (SOFT / desaturated) ----------------
% Two multigraph edge "types" (layers) -- using the light/desaturated
% counterparts of the original colors, same position in each gradient
\colorlet{EdgeTypeOne}{Cividis01}    % soft version of CividisDarkBlue -- 21 edges
\colorlet{EdgeTypeTwo}{ASPGrad12}    % soft version of ASPGold         --  7 edges

% Shared node styling (kept uniform across all three panels so the
% only visual variable across panels is the edge set/color)
\colorlet{NodeFill}{ASPMediumLightNavy}       % soft version of ASPNavy
\colorlet{NodeLabel}{ASPGrad01}      % soft version of ASPGold

\def\myEdgeOpacity{0.65}

% ---------------- Geometry (unchanged from original) ----------------
\def\myplotdimx{6cm}
\def\myplotdimy{6cm}
\def\my_gap_inter_plots{1.5cm}
\def\mynodesize{14}
\def\myrad{1.8cm}
\def\mylinewidth{1.5}




\begin{tikzpicture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% G R A P H   1 :  M U L T I G R A P H %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\path (0,0)  coordinate (caux1);

\SetDefaultUnit{pt}

\path (caux1)++(1*\myrad,0*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={ color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{1}, opacity=0.9,fontsize=\normalsize]{A}

\path (caux1)++(0.7071*\myrad ,0.7071*\myrad )  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={ color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{2}, opacity=0.9,fontsize=\normalsize]{B}

\path (caux1)++(0*\myrad , 1*\myrad )  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{3}, opacity=0.9,fontsize=\normalsize]{C}

\path (caux1)++(-0.7071*\myrad,0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{4}, opacity=0.9,fontsize=\normalsize]{D}

\path (caux1)++(-1.0000*\myrad,0*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{5}, opacity=0.9,fontsize=\normalsize]{E}

\path (caux1)++(-0.7071*\myrad,-0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{6}, opacity=0.9,fontsize=\normalsize]{F}

\path (caux1)++(0*\myrad,-1*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{7}, opacity=0.9,fontsize=\normalsize]{G}

\path (caux1)++(0.7071*\myrad,-0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{8}, opacity=0.9,fontsize=\normalsize]{H}

% ---- Type-1 edges (21) ----
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(B);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(C);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(D);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(C);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(D);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(E);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](C)(D);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](C)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](C)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](D)(E);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](D)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](D)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](E)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](E)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](F)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](G)(H);

% ---- Type-2 edges (7) ----
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](A)(E);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](B)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](C)(E);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](C)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](D)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](E)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](F)(H);

\path (caux1)++(0,-1.3*\myrad) coordinate (clabel1);
\node at (clabel1) {\color{black} $\ccalM = (\ccalV, \{\ccalE_r,w_{r}\}_{r=1}^{2})$};


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% G R A P H   2 :  T Y P E   1  O N L Y %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\path (4*\my_gap_inter_plots, 0)  coordinate (caux1);

\SetDefaultUnit{pt}

\path (caux1)++(1*\myrad,0*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{1}, opacity=0.9,fontsize=\normalsize]{A}

\path (caux1)++(0.7071*\myrad ,0.7071*\myrad )  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{2}, opacity=0.9,fontsize=\normalsize]{B}

\path (caux1)++(0*\myrad , 1*\myrad )  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{3}, opacity=0.9,fontsize=\normalsize]{C}

\path (caux1)++(-0.7071*\myrad,0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{4}, opacity=0.9,fontsize=\normalsize]{D}

\path (caux1)++(-1.0000*\myrad,0*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{5}, opacity=0.9,fontsize=\normalsize]{E}

\path (caux1)++(-0.7071*\myrad,-0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{6}, opacity=0.9,fontsize=\normalsize]{F}

\path (caux1)++(0*\myrad,-1*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{7}, opacity=0.9,fontsize=\normalsize]{G}

\path (caux1)++(0.7071*\myrad,-0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{8}, opacity=0.9,fontsize=\normalsize]{H}

% ---- Type-1 edges only (21) ----
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(B);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(C);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(D);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](A)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(C);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(D);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(E);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](B)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](C)(D);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](C)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](C)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](D)(E);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](D)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](D)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](E)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](E)(H);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](F)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeOne,opacity=\myEdgeOpacity](G)(H);

\path (caux1)++(0,-1.3*\myrad) coordinate (clabel2);
\node at (clabel2) {\color{EdgeTypeOne} $G_1 = (\ccalV, \ccalE_1, w_{1})$};


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% G R A P H   3 :  T Y P E   2  O N L Y %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\path (8*\my_gap_inter_plots, 0)  coordinate (caux1);

\SetDefaultUnit{pt}

\path (caux1)++(1*\myrad,0*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{1}, opacity=0.9,fontsize=\normalsize]{A}

\path (caux1)++(0.7071*\myrad ,0.7071*\myrad )  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{2}, opacity=0.9,fontsize=\normalsize]{B}

\path (caux1)++(0*\myrad , 1*\myrad )  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{3}, opacity=0.9,fontsize=\normalsize]{C}

\path (caux1)++(-0.7071*\myrad,0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{4}, opacity=0.9,fontsize=\normalsize]{D}

\path (caux1)++(-1.0000*\myrad,0*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{5}, opacity=0.9,fontsize=\normalsize]{E}

\path (caux1)++(-0.7071*\myrad,-0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{6}, opacity=0.9,fontsize=\normalsize]{F}

\path (caux1)++(0*\myrad,-1*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{7}, opacity=0.9,fontsize=\normalsize]{G}

\path (caux1)++(0.7071*\myrad,-0.7071*\myrad)  coordinate (caux2);
\gettikzy{(caux2)}{\ay};	\gettikzx{(caux2)}{\ax};
\Vertex[x=\ax, y=\ay, style={color=NodeFill},size=\mynodesize,label=\textcolor{NodeLabel}{8}, opacity=0.9,fontsize=\normalsize]{H}

% ---- Type-2 edges only (7) ----
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](A)(E);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](B)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](C)(E);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](C)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](D)(F);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](E)(G);
\Edge[lw=\mylinewidth,color=EdgeTypeTwo,opacity=\myEdgeOpacity](F)(H);

\path (caux1)++(0,-1.3*\myrad) coordinate (clabel3);
\node at (clabel3) {\color{EdgeTypeTwo} $G_2 = (\ccalV, \ccalE_2, w_{2})$};

\end{tikzpicture}




